Can Image Generators Hold a Scene Together When Space Is Broken Apart?

Image generators are good at drawing scenes in which things that belong together appear next to each other. In almost every image they generate, and in almost every benchmark used to evaluate these images, "belonging to the same whole" and "adjacent to each other" go together. Therefore, we cannot know whether the model truly grasps the scene as a whole, or simply makes each part connect with its adjacent parts. We propose GJBench to disentangle the two. It requires the model to draw a scene as a scattered jigsaw puzzle: an image is cut into interlocking pieces, then moved apart and rotated. Thus, the spatial plausibility of the scene exists only in how these pieces collectively point to a whole. The model may have a reference image, a target layout, both, or neither. We separately evaluate three requirements: whether the scene is broken down into a specified number of separate pieces, whether the pieces interlock, and whether the pieces can reconstruct the reference scene. While every open and closed model we evaluated could draw these scenes well as a whole, none could keep them together as scattered puzzle pieces, and the three requirements categorized failures into different patterns. The models draw separate pieces but miscount them in different ways, and unless their outlines are provided, the pieces rarely interlock, and their content does not reconstruct the reference image. We also found that the target layout helps the puzzle pieces fit together, while the reference image improves neither their count nor their fit. These findings show that keeping a scene continuous across space that the canvas no longer shows remains an open problem for image generators.

==> generated/tab_v3_main_body.tex <==
GPT Image 2.6 & .98 & .98 & .94 & .74 & .73 & .74 & .38 & .45 & .49 \\
Nano Banana 2.1 & .95 & .83 & .45 & .63 & .63 & .57 & .38 & .45 & .48 \\
Muse Image 1.0 & .74 & .72 & .50 & .56 & .64 & .65 & .33 & .40 & .44 \\
Qwen-Image-2.1 & .79 & .76 & .65 & .51 & .51 & .50 & .33 & .33 & .37 \\
FLUX 3 Image Klein & .73 & .67 & .39 & .28 & .34 & .33 & .31 & .35 & .39 \\
\midrule
Control & 1.00 & 1.00 & 1.00 & .95 & .94 & .89 & .94 & .93 & .94 \\

